Search for electric dipole moments

Searches for permanent electric dipole moments of fundamental particles and systems with spin are the experiments most sensitive to new CP violating physics and a top priority of a growing international community. We briefly review the current status of the field emphasizing on the charged leptons and lightest baryons.

==> packages.tex <==
\usepackage[T1]{fontenc}
\usepackage{aas_macros}
%\usepackage{fourier}
\usepackage{lmodern}
%\usepackage[scaled=0.875]{helvet} % sansSerif
%\renewcommand{\ttdefault}{lmtt} %tt   font for typewriter
%\usepackage[official,right]{eurosym}
\usepackage{textcomp}   % provides proper micro- and degree-symbol
\usepackage{gensymb}
%\usepackage[latin1]{inputenc}
\usepackage[english]{babel}
%\usepackage[dvipsnames,pdftex]{xcolor}
%\usepackage[pdftex]{graphicx,epsfig}
\usepackage{rotating}
%\usepackage{eso-pic}
%\usepackage{wrapfig}
%\usepackage{epsf}
%\usepackage{fancybox}
%\usepackage{amsmath,amsthm,amssymb,amsfonts} %% too many math alphabets! DRi
%\usepackage{amsmath,amsthm}
%\usepackage{dsfont}\let\mathbb\mathds
%\usepackage[hyphens]{url}
\usepackage[breaklinks=true,hidelinks]{hyperref}
%\usepackage[breaklinks=true]           {hyperref}   %better for final layouting: to find link to figures in text
%\usepackage[section]{placeins} %allows to have unlimited floats
%\usepackage{needspace}
%\usepackage{setspace}
%\usepackage[suffix='']{epstopdf}
%\usepackage{epigraph}
\usepackage{tabularx}
%\usepackage[font=small,margin=1cm]{caption}
%\usepackage{subfig}
%\usepackage[percent]{overpic}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{MnSymbol}
\usepackage[tight,nice]{units}
\usepackage{xspace}
\usepackage{pbox}
%\usepackage{isotope}
%\usepackage{tikz} %added for Victor
%\usepackage[markers,nolists]{endfloat} %zc, for editing 2013-12-23
%\usepackage{float}%added for Victor
\usepackage{siunitx}%added by Martin
%\usepackage{enumitem}%added by jochen to get rid of space above itemize and enumerate environments


% we get error:  "PDF icnlusion  multiple pdfs with page group included in a single page"'
%usepackage{silence }  does not help for  this  (because it is pdflatex low level??) 
% maybe use  gs  on those files  (all pdf with transparency,  including those via gnuplot pdfcairo)
%http://tex.stackexchange.com/questions/76273/multiple-pdfs-with-page-group-included-in-a-single-page-warning
%or we can use LuaLaTex  (but then we should get rid of package epstopdf
%or is it my pdflatex?  MiKTeX-pdfTeX 2.9.4902 (1.40.14) (MiKTeX 2.9 64-bit)     22.06.2013  22:16

